GenPose: Generative Category-level Object Pose Estimation via Diffusion Models

Object pose estimation plays a vital role in embodied AI and computer vision, enabling intelligent agents to comprehend and interact with their surroundings. Despite the practicality of category-level pose estimation, current approaches encounter challenges with partially observed point clouds, known as the multihypothesis issue. In this study, we propose a novel solution by reframing categorylevel object pose estimation as conditional generative modeling, departing from traditional point-to-point regression. Leveraging score-based diffusion models, we estimate object poses by sampling candidates from the diffusion model and aggregating them through a two-step process: filtering out outliers via likelihood estimation and subsequently mean-pooling the remaining candidates. To avoid the costly integration process when estimating the likelihood, we introduce an alternative method that trains an energy-based model from the original score-based model, enabling end-to-end likelihood estimation. Our approach achieves state-of-the-art performance on the REAL275 dataset, surpassing 50% and 60% on strict 5d2cm and 5d5cm metrics, respectively. Furthermore, our method demonstrates strong generalizability to novel categories sharing similar symmetric properties without fine-tuning and can readily adapt to object pose tracking tasks, yielding comparable results to the current state-of-the-art baselines.

==> RebuttalTables/eps.tex <==
\begin{tabular}{cc|cccc}
\toprule
eps                    & Ranking & $5^{\circ}2$cm  & $5^{\circ}5$cm  & $10^{\circ}2$cm  &$10^{\circ}5$cm  \\ \toprule
\multirow{2}{*}{1e-5}  & Energy  & \textbf{52.4(\blod{\scriptsize{2.5$\uparrow$}})}   & \textbf{61.2(\blod{\scriptsize{1.7$\uparrow$}})}   & \textbf{72.8(\blod{\scriptsize{3.7$\uparrow$}})}    & \textbf{84.2(\blod{\scriptsize{2.5$\uparrow$}})}   \\
                       & Rondom  & 49.9            & 59.5            & 69.1             & 81.7            \\ \midrule
\multirow{2}{*}{1e-2}  & Energy  & \textbf{49.7(\blod{\scriptsize{4.9$\uparrow$}})}   & \textbf{60.9(\blod{\scriptsize{2.6$\uparrow$}})}   & \textbf{69.4(\blod{\scriptsize{6.1$\uparrow$}})}    & \textbf{84.2(\blod{\scriptsize{2.7$\uparrow$}})}   \\     
                       & Random  & 44.8            & 58.3            & 63.3             & 81.5            \\ \midrule
\multirow{2}{*}{2e-1}  & Energy  & \textbf{33.5(\blod{\scriptsize{16.5$\uparrow$}})}   & \textbf{59.3(\blod{\scriptsize{4.7$\uparrow$}})}   & \textbf{47.2(\blod{\scriptsize{21.9$\uparrow$}})}    & \textbf{83.5(\blod{\scriptsize{3.0$\uparrow$}})}   \\       
                       & Random  & 17.0            & 54.6            & 25.3             & 80.5            \\ \hline
\end{tabular}

==> RebuttalTables/novel_category.tex <==
\begin{tabular}{c|c|cccc}
\toprule
Category    & Method     & $5^\circ$2cm                  & $5^\circ$5cm                   & $10^\circ$2cm                   & $10^\circ$5cm                    \\ \midrule
            & SAR-Net    & 58.1/36.4                     & 66.0/47.3                      & 83.7/59.4                       & 93.6/81.5                        \\
bowl        & RBP-Pose   & 75.4/0.0                      & 81.7/6.9                       & 92.1/0.1                        & \textbf{100.0}/30.7              \\
            & Ours       & \textbf{85.7}/\textbf{64.5}   & \textbf{92.6}/\textbf{72.5}    & \textbf{93.1}/\textbf{87.2}     & \textbf{100.0}/\textbf{98.6}     \\ \midrule
            & SAR-Net    & 43.5/11.7                     & 54.0/23.0                      & 61.3/33.6                       & 79.8/68.0                        \\
bottle      & RBP-Pose   & 38.7/4.3                      & 43.5/5.8                       & 76.4/24.7                       & 89.8/29.7                        \\
            & Ours       & \textbf{53.6}/\textbf{39.0}   & \textbf{62.0}/\textbf{53.2}    & \textbf{81.4}/\textbf{73.6}     & \textbf{92.7}/\textbf{94.6}      \\ \midrule  
            & SAR-Net    & 32.2/7.3                      & 62.2/52.3                      & 52.5/12.1                       & 92.9/87.9                        \\
can         & RBP-Pose   & 53.5/0.8                      & 67.1/21.0                      & 78.8/2.6                        & 96.3/61.7                        \\  
            & Ours       & \textbf{73.2}/\textbf{62.5}   & \textbf{81.2}/\textbf{74.0}    & \textbf{88.8}/\textbf{81.6}     & \textbf{99.8}/\textbf{99.7}      \\ \bottomrule
\end{tabular}

==> RebuttalTables/score_vs_energy.tex <==
\begin{tabular}{cc|cccc}
\toprule
Sampling & Ranking    & $5^{\circ}2$cm   & $5^{\circ}5$cm   & $10^{\circ}2$cm  & $10^{\circ}5$cm  \\ \midrule
Score            & Energy             & \textbf{52.4}    & \textbf{61.2}    & \textbf{72.8}    & \textbf{84.2}      \\
Energy           & Energy             & 40.9             & 53.1             & 60.5             & 78.3               \\ \bottomrule
\end{tabular}

==> RebuttalTables/steps.tex <==
\begin{tabular}{cc|cccc}
\toprule
steps                  & Ranking & $5^{\circ}2$cm  & $5^{\circ}5$cm  & $10^{\circ}2$cm  &$10^{\circ}5$cm  \\ \toprule
\multirow{2}{*}{500}   & Energy  & \textbf{52.4(\blod{\scriptsize{2.5$\uparrow$}})}   & \textbf{61.2(\blod{\scriptsize{1.7$\uparrow$}})}   & \textbf{72.8(\blod{\scriptsize{3.7$\uparrow$}})}    & \textbf{84.2(\blod{\scriptsize{2.5$\uparrow$}})}    \\
                       & Rondom  & 49.9            & 59.5            & 69.1             & 81.7            \\ \midrule
\multirow{2}{*}{10}    & Energy  & \textbf{48.9(\blod{\scriptsize{6.9$\uparrow$}})}   & \textbf{60.6(\blod{\scriptsize{2.5$\uparrow$}})}   & \textbf{68.5(\blod{\scriptsize{9.2$\uparrow$}})}    & \textbf{84.2(\blod{\scriptsize{2.5$\uparrow$}})}    \\     
                       & Random  & 42.0            & 58.1            & 59.3             & 81.7            \\ \midrule
\multirow{2}{*}{5}     & Energy  & \textbf{40.8(\blod{\scriptsize{13.5$\uparrow$}})}   & \textbf{59.5(\blod{\scriptsize{3.2$\uparrow$}})}   & \textbf{57.8(\blod{\scriptsize{18.4$\uparrow$}})}    & \textbf{83.8(\blod{\scriptsize{2.7$\uparrow$}})}   \\       
                       & Random  & 27.3            & 56.3            & 39.6             & 81.1            \\ \hline
\end{tabular}

==> RebuttalTables/weighted_mean_pooling.tex <==
\begin{tabular}{c|cccc}
\toprule
Aggregation      & $5^{\circ}2$cm   & $5^{\circ}5$cm   & $10^{\circ}2$cm  & $10^{\circ}5$cm     \\ \midrule
Mean pooling     & \textbf{52.4}    & \textbf{61.2}    & \textbf{72.8}    & \textbf{84.2}       \\
Weighted pooling & 47.1             & 59.3             & 65.1             & 81.7                \\ \bottomrule
\end{tabular}
